ViSTa Dataset: Do vision-language models understand sequential tasks?

Using vision-language models (VLMs) as reward models in reinforcement learning holds promise for reducing costs and improving safety. So far, VLM reward models have only been used for goal-oriented tasks, where the agent must reach a particular final outcome. We explore VLMs' potential to supervise tasks that cannot be scored by the final state alone. To this end, we introduce ViSTa, a dataset for evaluating Vision-based understanding of Sequential Tasks. ViSTa comprises over 4,000 videos with step-by-step descriptions in virtual home, Minecraft, and real-world environments. Its novel hierarchical structure -- basic single-step tasks composed into more and more complex sequential tasks -- allows a fine-grained understanding of how well VLMs can judge tasks with varying complexity. To illustrate this, we use ViSTa to evaluate state-of-the-art VLMs, including CLIP, ViCLIP, and GPT-4o. We find that, while they are all good at object recognition, they fail to understand sequential tasks, with only GPT-4o achieving non-trivial performance.

==> assets/obj_recognition_habitat.tex <==
\begin{tikzpicture}[
scale=1
]

\definecolor{myred}{HTML}{da1916}
\definecolor{myblue}{HTML}{437eb7}
\definecolor{mygreen}{HTML}{59ac49}

\begin{axis}[
ymin=0,
ymax=1,
scale=1,
ylabel=Average Macro F1,
ylabel style={align=center},
ytick style={draw=none},
xtick style={draw=none},
y tick label style={font=\normalsize},
x tick label style={left,
font=\normalsize},
axis line style={draw=none},
tick align=outside,
major tick length=1.75,
ymajorgrids,
extra y ticks=0,
extra y tick labels=,
extra y tick style={grid=major,
major grid style={color=black}},
xmin=-0.5,
xmax=2.5,
x=20pt,
y=100pt,
bar width=0.75,
xticklabels={{CLIP},
{\gptfour}o,
{\viclip}},
x tick label style={rotate=-90, anchor=west},
xtick={0,
1,
2}
]
\addplot[ybar, fill=myred, opacity=0.5, draw=myred, very thickes {(0.7746031740,6031745,0)};
\addplot[ybar, fill=myblue, opacity=0.5, draw=myblue, very thickes {(0.8857142851,7142857,1)};
\addplot[ybar, fill=mygreen, opacity=0.5, draw=mygreen, very thickes {(0.5555555552,5555555,2)};
\draw[densely dotted, thick, color=black] (-1,0.16666666666666666) -- (4,0.16666666666666666);
\end{axis}
\normalsize
\node (title) at (0.5*100pt, 110pt) [above] {Objects -- Habitat};
\end{tikzpicture}


==> assets/obj_recognition_real.tex <==
\begin{tikzpicture}[
scale=1
]

\definecolor{myred}{HTML}{da1916}
\definecolor{myblue}{HTML}{437eb7}
\definecolor{mygreen}{HTML}{59ac49}

\begin{axis}[
ymin=0,
ymax=1,
scale=1,
ylabel=Average Macro F1,
ylabel style={align=center},
ytick style={draw=none},
xtick style={draw=none},
y tick label style={font=\normalsize},
x tick label style={left,
font=\normalsize},
axis line style={draw=none},
tick align=outside,
major tick length=1.75,
ymajorgrids,
extra y ticks=0,
extra y tick labels=,
extra y tick style={grid=major,
major grid style={color=black}},
xmin=-0.5,
xmax=2.5,
x=20pt,
y=100pt,
bar width=0.75,
xticklabels={{CLIP},
{\gptfour}o,
{\viclip}},
x tick label style={rotate=-90, anchor=west},
xtick={0,
1,
2
}
]
\addplot[ybar, fill=myred, opacity=0.5, draw=myred, very thick] coordinates {(0, 1.0)};
\addplot[ybar, fill=myblue, opacity=0.5, draw=myblue, very thick] coordinates {(1, 1.0)};
\addplot[ybar, fill=mygreen, opacity=0.5, draw=mygreen, very thick] coordinates {(2, 1.0)};
\draw[densely dotted, thick, color=black] (-1, 0.16666666666666666) -- (3, 0.16666666666666666);
\end{axis}
\normalsize
\node (title) at (0.5*100pt, 110pt) [above] {Objects -- Real};
\end{tikzpicture}

